ARIST: An Effective API Argument Recommendation Approach

Learning and remembering to use APIs are difficult. Several techniques have been proposed to assist developers in using APIs. Most existing techniques focus on recommending the right API methods to call, but very few techniques focus on recommending API arguments. In this paper, we propose ARIST, a novel automated argument recommendation approach which suggests arguments by predicting developers' expectations when they define and use API methods. To implement this idea in the recommendation process, ARIST combines program analysis (PA), language models (LMs), and several features specialized for the recommendation task which consider the functionality of formal parameters and the positional information of code elements (e.g., variables or method calls) in the given context. In ARIST, the LMs and the recommending features are used to suggest the promising candidates identified by PA. Meanwhile, PA navigates the LMs and the features working on the set of the valid candidates which satisfy syntax, accessibility, and type-compatibility constraints defined by the programming language in use. Our evaluation on a large dataset of real-world projects shows that ARIST improves the state-of-the-art approach by 19% and 18% in top-1 precision and recall for recommending arguments of frequently-used libraries. For general argument recommendation task, i.e., recommending arguments for every method call, ARIST outperforms the baseline approaches by up to 125% top-1 accuracy. Moreover, for newly-encountered projects, ARIST achieves more than 60% top-3 accuracy when evaluating on a larger dataset. For working/maintaining projects, with a personalized LM to capture developers' coding practice, ARIST can productively rank the expected arguments at the top-1 position in 7/10 requests.

==> 4.ArgRec/4.2.filtering_candidates_Kien.tex <==

\subsection{Filtering Candidates}

%-----------------------------------------------
% General objective: lọc các candidates phù hợp để chuyển cho global models
% Lý do: có rất nhiều valid candidates được sinh ra, đặc biệt nếu expected type là Object -> ảnh hưởng đến performance của các neural network models
% Process: (1) Giữ lại các candidates có khả năng phù hợp cao: gồm có public static parameter similarity và classes recentness; (2) sử dụng nested-cache model để ranking các candidates (được giữ lại); (3) để tăng độ chính xác thì kết hợp với lexsim; (4) giữ lại top-k candidates và chuyển sang cho global model
%
% 1. Giữ lại các candidates phù hợp:
%       1.1. Đưa ra một số rules và thống kê trên 1 tập nhỏ dữ liệu -> cover được targets ở hầu hết các cases -> với target là object, strings, primitive, chỉ giữ lại các candidates theo rules này
%      1.2. Theo rule trên có 2% cases bị miss targets->investigate thấy các cases này rơi vào trường hợp members of the same classes được dùng trong cùng context -> sử dụng tính recentness
%       Có thể cân nhắc coi 1.2 là 1 rule của phần 1.1 và làm tương tự như các rules khác trong phần này.
% 2. Ranking candidate bằng nested-cache model
%       - Vì sao dùng nested-cache
%       - Cấu hình
% 3. lexism
%       - mục tiêu tăng độ chính xác
%       - lý do: arguments thường rất giống hoặc rất khác formal parameters
%       - Kết hợp với score của nested-cache model như thế nào? lý do?
% 4. Giữ lại top-k candidates và chuyển global model
%-----------------------------------------------






%Kien, create a separated file
\label{sec:filter_cand}
There can be a large number of type-corrected candidates, especially when the type of target is \texttt{Object} or other common types, such as \texttt{String} or \texttt{int}. In fact, large projects such as Netbeans or Eclipse can have more than 100k accessible variables of type \texttt{Object}. While neural network models, such as RNN or LSTM, can capture long context information, they often takes considerable amount of time in order to produce their output. In contrast, \emph{N}-gram models, while not able to capture long context, can still produce positive result \cite{nestedcache} by making use of source code hierarchy. To combine the strength of these two types of model, we have come at the following approach: First, we filter the possibly large number of valid candidates by combining language models with source code features, including \emph{Lexical similarity}, \emph{Class recentness} and \emph{Public static parameter similarity} (details at the following sections). The model that filters candidates will be refered as \emph{local model}. The correct candidate might appear in this list, but it may not be at the top position. That's why we need to use another model that can effectively reorganize the small number of candidates. This model can be of any type of model. In this paper, we use GPT-2 - a ........................................................... We will refer to this model as \emph{global model}. In this section, we will describe the local model, along with the techniques used to filter candidates.
\subsubsection{Local language model}
We adopt the nested-cache model \cite{nestedcache} to build language models to rank candidates at this step. This model is able to capture source code locality. The nested model learns code patterns in a nested, scoped fashion, while the cache model tracks the local change within a single source file. We use the Jelinek-Mercer (JM) smoothing with a fixed confidence of 0.5 and \emph{n} = 6 for the length of \emph{N}-grams.
\subsubsection{Lexical similarity}
In practice, the actual parameters and the formal parameters are often significantly similar or completely dissimilar in terms of lexical tokens~\cite{liu2016nomen}. 
We also validated this statement in the two projects, Eclipse and Netbeans. 
It shows that 68.24\% actual parameters and formal parameters are totally similar and 
22.33\% of them are completely different. This means that among the generated candidates, \textit{the more lexical similar to the formal parameter a candidate is, the higher probability it is the expected actual parameter}.\\

To improve the accuracy of the nested cache models, we also take into account the lexical similarity (lexsim) of the actual parameters and the corresponding formal parameters. Particularly, we leverage the formula proposed by Liu et al.~\cite{liu2016nomen} to calculate the similarity of a candidate ($c$) and the corresponding formal parameter ($p$), as follows:


\begin{equation}
lexsim(c, p) =\frac{|comterms(c,p)| + |comterms(c,p)|}{|terms(c)| + |terms(p)|}
\end{equation}

In this formula, 
\begin{itemize}
  \item \textbf{\textit{terms(s)}}: The decomposition of \textit{s}, based on underscores and capital letters.
  \item \textbf{\textit{comterms(n1, n2):}} is the longest subsequence of \textit{terms(n1)} and \textit{terms(n2)}.
\end{itemize}


\subsubsection{Public static parameter filtering}
\label{staticparamfilter}
Large projects, such as Netbeans or Eclipse, may have a large number of public static variables from multiple sources, including the JRE, the libraries used in the project, and the project itself. These variables are usually config options. Public static parameters account for 5\%-10\% of argument usage. Most public static variable are of type String, and int (or Integer) type, as in \ref{table:pscountstat}. This poses a threat to the language model performance. The large number of candidates can also produce a lot of noise. We notice that, most of the times, if the target argument is a public static variable, it often has some similarities to its surrounding context. So to reduce the number of noisy public static candidates, we only keep candidates that satisfy at least one of the following conditions:
\begin{itemize}
\item Candidate has at least one similar subtoken (by camel case or snake case convention) with one of the followings:
  \begin{itemize}
    \item Caller method name, such as \emph{m1} in Listing \ref{environmentt}
    \item Callee method name, such as \emph{m2} in Listing \ref{environmentt}
    \item Caller object name, such as \emph{a} in Listing \ref{environmentt}
    \item Caller object type, such as \emph{Object1} in Listing \ref{environmentt}
  \end{itemize}
  Note that we only consider alphanumeric subtokens, since a variable may have punctuations in its lexical representation.
\item It is a boundary variables, such as \texttt{Integer.MAX\_VALUE}
\item It is in the package scope
\item It is a member of a parent class
\item It is a member of a class that was previously used in the same source file.
\end{itemize}

These rules are only applied if target is of type \emph{Object}, \emph{String} or numeric types, since the number of public static variables for user-defined types are significantly smaller.

Note that the actual target may not satisfy any conditions above. In fact, after filtering, ~1.8\% of argument usages in Netbeans, and ~2.6\% of argument usages in Eclipse lost the target candidate, but the number of public static candidates is reduced by an average of ~75\%, which is significant. So we can reduce a lot of noise without sacrificing too much accuracy.

\begin{lstlisting}[language=Java,label=environmentt,caption=Environment]
public m1(){
  Object1 a = new Object1();
  Object2 b = a.m2();
}
\end{lstlisting}


\begin{table}[]
\centering
\caption{Number of public static variables on common types on JRE and large projects}
\label{table:pscountstat}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Project & Total & String & int & bool\\\hline
JRE & 31,971 & 5,914 & 9,829 & 1,542\\
Eclipse & 74,405 & 41,446 & 15,656 & 2,283\\
Netbeans & 52,313 & 28,987 & 5,139 & 2,922\\\hline
% Eclipse & 106,376 & 47,360 & 25,485 & 6,100 & 3,825\\
% Netbeans & 84,284 & 34,901 & 14,968 & 3,193 & 4,464\\\hline
\end{tabular}
\end{table}

% \subsubsection{Classes recentness}
% In certain cases, members of the same class are used consecutively in the same source file (i.e. switch statement), as in the following simplified code snippet from Netbeans:
% \begin{lstlisting}[language=Java,label=classRecentness,caption=Class recentness example]
% private static DocFinder getFinder(...) {
%     ...
%     b = searchProps.get(EditorFindSupport.FIND_MATCH_CASE);
%     boolean matchCase = (b != null && b.booleanValue());
%     b = searchProps.get(EditorFindSupport.FIND_SMART_CASE);
%     boolean smartCase = (b != null && b.booleanValue());
%     b = searchProps.get(EditorFindSupport.FIND_WHOLE_WORDS);
%     boolean wholeWords = (b != null && b.booleanValue());
%     ...
% }
% \end{lstlisting}
% To make use of this, we store the all classes of expected parameter in the current source file. Then all public static, type-corrected members of these classes are added to candidate list. These candidates are kept as-is, not filtered by the \label{staticparamfilter} rule. 
% This work like cache model. Recent classes will be cleared when switching to a new file.
\subsubsection{Filtering process}
We filter the public static parameter, according the the \ref{staticparamfilter} rules. Then we add parameters to candidate list according the \emph{recentness of classes} rules. Then each candidate are scored by the product of its lexsim score and the nested cache model's probability. Top-\emph{k} candidates with highest score are forwarded to the next step. The \emph{k} parameter should be small enough to not hinder the overall performance, since the global model might take some time to score a candidate. The \emph{k} should also being large enough to not missing out the target. For these reasons, we choose \emph{k} to be 20.
%

==> 4.ArgRec/4.2.filtering_candidates_bk.tex <==

\subsection{Reducing Candidates}

%-----------------------------------------------
% General objective: lọc các candidates phù hợp để chuyển cho global models
% Lý do: có rất nhiều valid candidates được sinh ra, đặc biệt nếu expected type là Object -> ảnh hưởng đến performance của các neural network models
% Process: (1) Giữ lại các candidates có khả năng phù hợp cao: gồm có public static parameter similarity và classes recentness; (2) sử dụng nested-cache model để ranking các candidates (được giữ lại); (3) để tăng độ chính xác thì kết hợp với lexsim; (4) giữ lại top-k candidates và chuyển sang cho global model
%
% 1. Giữ lại các candidates phù hợp:
%       1.1. Đưa ra một số rules và thống kê trên 1 tập nhỏ dữ liệu -> cover được targets ở hầu hết các cases -> với target là object, strings, primitive, chỉ giữ lại các candidates theo rules này
%      1.2. Theo rule trên có 2% cases bị miss targets->investigate thấy các cases này rơi vào trường hợp members of the same classes được dùng trong cùng context -> sử dụng tính recentness
%       Có thể cân nhắc coi 1.2 là 1 rule của phần 1.1 và làm tương tự như các rules khác trong phần này.
% 2. Ranking candidate bằng nested-cache model
%       - Vì sao dùng nested-cache
%       - Cấu hình
% 3. lexsim
%       - mục tiêu tăng độ chính xác
%       - lý do: arguments thường rất giống hoặc rất khác formal parameters
%       - Kết hợp với score của nested-cache model như thế nào? lý do?
% 4. Giữ lại top-k candidates và chuyển global model
%-----------------------------------------------






%Kien, create a separated file
\label{sec:filter_cand}
For an argument, there could be a large number of type-valid candidates, especially, when the expected type of the corresponding formal parameter is \texttt{Object} or another primary data type such as \texttt{String} or \texttt{int}. For instance, in large projects such as Eclipse, there are more than 100K accessible and type-valid candidates per case whose expected type is  \texttt{Object}. 
Indeed, in these type-valid candidates, there are an enormous number of candidates which are irrelevant to the coding context. Furthermore, with such large amount of candidates, a recommendation system often takes times and also struggles to figure out the most suitable one. Therefore, \textit{those less relevant candidates should be filtered out to ensure the performance of the ranking model.}

In this work, we combine source code features and a light weight language model to filter candidates. Specifically, arguments often expose their suitableness with the coding contexts in some sort of similarities. Therefore, only candidates which are similar to the coding contexts are kept, the others are removed. After that, we use a light weight LM to select top-k most suitable candidates for further ranking.



\subsubsection{Similarity of arguments and coding contexts}
\label{staticparamfilter}
We hypothesize that arguments often have relations with the coding context in terms of scopes and/or names.
Specifically, the arguments are frequently similar to the caller/called method names or object names. 
For example in Fig.~\ref{fig:example_code}, at line 10, the called method name is 
\texttt{setName} and the corresponding argument also contains token \texttt{Name}. Also, at line 14, the called method name is \texttt{setAccess} and the token \texttt{Access} is contained in the argument name as well. 
Therefore, among the generated type-valid candidates, we only keep candidates which satisfy one of these following rules:

\begin{itemize}
    %Stat
    \item Having at least one similar subtoken (case insensitive) with one of the following items: caller method name, called method name, caller object name, or caller object type. Note that we only consider subtokens comprising of letters and digits.
    \item Is a boundary variable (max/min)
    %Scope
    \item Is a member of the class/parent classes of the coding context
    \item Is declared in the same package scope of the coding context
    %Reuse
    \item Is a member of a class whose other members are used in the coding context.
\end{itemize}


\begin{figure}
    \centering
    \small
    \lstinputlisting[language=Java]{images/example_filtering.m}
   \caption{An example in project Netbeans}
    \label{fig:example_filtering}
\end{figure}{}


Fig.~\ref{fig:example_filtering} shows an example in the project Netbeans. At line 3, it is expected an arguments type \texttt{Object}. There are 34901 valid public static candidates in total. By applying our proposed filtering rules, only 3970 of them are kept for further ranking. Specially, they are (note that some candidates may satisfy multiple rules):
\begin{itemize}
    \item 3562 candidates which contain similar subtokens with the caller method name (\texttt{isBackgroundDrawing}), the called method name (\texttt{getProp}), the caller object name (\texttt{b}), and the caller object type (\texttt{Boolean}), such as \texttt{Watch.PROP\_VALUE},  \texttt{AnnotationDesc.PROP\_ANNOTATION\_TYPE}, \texttt{Constants.COLOR\_TAB\_BACKGROUND}, etc. 
    \item 191 candidates which are in same package (\texttt{org.netbeans.editor}) or in the same class/parent class (\texttt{AnnotationTypes}) with the coding context. For example, \texttt{PROP\_BACKGROUND\_DRAWING}, \texttt{PROP\_BACKGROUND\_GLYPH\_ALPHA}, etc.
    \item 314 candidates are boundary values, such as \texttt{Integer.MAX\_VALUE}
\end{itemize}


To verify our hypothesis, we examined \textbf{35281} cases in project Netbeans. Our investigation result shows that there are 2753 cases which have arguments satisfied our proposed rules. Importantly, by applying these filtering rules, a large number of noise has been removed (91.5\% of candidates) without sacrificing too much accuracy.
Specially: 
\begin{itemize}
    \item 2530 cases where the arguments are similar to caller/called method name, object name, object type
    \item 141 cases where the arguments are boundary values
    \item 969 cases where the arguments are variables/members in the class/parent classes of the coding context
    \item 175 cases where the arguments are members of the classes in the same package with the coding context
    \item 1845 cases where arguments come from classes which are already used in the coding context
\end{itemize}


%Note that we only consider alphanumeric subtokens, since a variable may have punctuations in its lexical representation.


% These rules are only applied if target is of type \emph{Object}, \emph{String} or numeric types, since the number of public static variables for user-defined types are significantly smaller.

% Note that the actual target may not satisfy any conditions above. In fact, after filtering, ~1.8\% of argument usages in Netbeans, and ~2.6\% of argument usages in Eclipse lost the target candidate, but the number of public static candidates is reduced by an average of ~75\%, which is significant. So we can reduce a lot of noise 




% \begin{table}[]
% \centering
% \caption{Number of public static variables on common types on JRE and large projects}
% \label{table:pscountstat}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Project & Total & String & int & bool\\\hline
% JRE & 31,971 & 5,914 & 9,829 & 1,542\\
% Eclipse & 74,405 & 41,446 & 15,656 & 2,283\\
% Netbeans & 52,313 & 28,987 & 5,139 & 2,922\\\hline
% % Eclipse & 106,376 & 47,360 & 25,485 & 6,100 & 3,825\\
% % Netbeans & 84,284 & 34,901 & 14,968 & 3,193 & 4,464\\\hline
% \end{tabular}
% \end{table}


\subsubsection{Local language model}
After filtering candidates based on comparing their scope/similarity with the caller/called name in the corresponding context, a large number of irreverent candidates are removed. However, the amount of remaining candidates per case is still very large. In order to continuously narrow down the search space, we select top-k most suitable candidates using a light weight LM, nested-cached model~\cite{nestedcache}.

Indeed, the nested-cache model is a count-based N-gram model therefore it is fast and it can work well with unlimited vocabulary. Moreover, its nested design helps to capture the source code locality which is an important characteristic in software program. For instance, method/class/variable names are often invented and used repeatedly in one scope, and never used elsewhere~\cite{bruch2009learning, tu2014localness}. 
%
Specially, the nested-cache model contains two parts: the nested model learns code patterns in a nested, scoped fashion and the cache model tracks the local change within a single source file. 
%
In this work, we use the Jelinek-Mercer (JM) smoothing with a fixed confidence of 0.5 and \emph{n} = 6 for the length of \emph{N}-grams.

\subsubsection{Lexical similarity}
In practice, the actual parameters and the formal parameters are often significantly similar or completely dissimilar in terms of lexical tokens~\cite{liu2016nomen}. 
We also validated this argument in the two projects, Eclipse and Netbeans. 
It shows that 68.24\% actual parameters and formal parameters are totally similar and 
22.33\% of them are completely different. This means that among the generated candidates, \textit{the more lexical similar to the formal parameter a candidate is, the higher probability it is the expected actual parameter}.\\

To improve the performance of the local model, we also take into account the lexical similarity (lexsim) of the candidates and the corresponding formal parameters. Particularly, we leverage the formula proposed by Liu et al.~\cite{liu2016nomen} to calculate the similarity of a candidate ($c$) and the corresponding formal parameter ($p$), as follows:


\begin{equation}
lexsim(c, p) =\frac{|comterms(c,p)| + |comterms(c,p)|}{|terms(c)| + |terms(p)|}
\end{equation}

In this formula, 
\begin{itemize}
  \item \textbf{\textit{terms(s)}}: The decomposition of \textit{s}, based on underscores and capital letters.
  \item \textbf{\textit{comterms(n1, n2):}} is the longest subsequence of \textit{terms(n1)} and \textit{terms(n2)}.
\end{itemize}



\subsubsection{Object Mapping}
\label{objectmapping}
An issue detected in our research progress is that when a parameter is declared by \texttt{java.lang.Object}, it can accept all candidates with any data type. This is the reason why there are so many test cases in which our method predicts a lot of candidates \~ 121K candidates.

When reviewing the test cases, we see some \texttt{java.lang.Object} parameters, those have the same name with type parameters on generic type\footnote{https://docs.oracle.com/javase/tutorial/java/generics/types.html}. For example, \texttt{java.util.HashMap}\footnote{https://docs.oracle.com/javase/8/docs/api/java/util/HashMap.html} class on Table. \ref{fig:hashmap} declares a method which is "containsKey" having one argument with Object as the data type. Besides, there is a parameter named "key", which has the same name as another parameter of method "put". However, that parameter from "put" has the data type "K", which is a type parameter of a generic type. In fact, the developer will only put into "containsKey" method with a key that has the same data type as those keys put to that object by the \texttt{put} method.

The idea is based on the previous usages of type argument generic type to compare and map to an \texttt{Object} parameter with the same name. Within JDK8 (8u74), we found 247 usage cases for mapping from \texttt{Object} to a type parameter of generic type. When applying that method to identifying valid candidates on Netbeans and Eclipse, the number of candidates from Object map with \texttt{Integer} reduces 44.5\%, and with \texttt{boolean} is 99.6\%. The number of candidates will reduce by over 99\% if the \texttt{Object} is mapped with a class not belonging to JDK. Overall, the number of candidates of Netbeans and Eclipse reduces 4.91\% on all test cases, and accuracy reduces by less than 0.01\%.



For summary, all the typed-valid and accessible candidates which are generated in the previous phase will be filtered according to the their similarities in terms of names and scopes with the corresponding coding context. After that, we evaluate their suitableness with the context by the nested-cache model and lexsim metric. Specially, the score of each candidate is measured by the \textit{product} of the model's predicted probability and the lexsim score. Finally, top-k candidates are further examined in the next phase.
The \emph{k} parameter should be small enough to not hinder the overall performance, since the global model might take some time to score a candidate. The \emph{k} should also being large enough to not missing out the target. For these reasons, we choose \emph{k} to be 20.
%

==> 4.ArgRec/4.3.ranking_candidates.tex <==
\subsection{Ranking Candidates}
%Tan, create a separated file

==> 4.ArgRec/tan_bk.tex <==

\subsection{Ranking Candidates}
% Ở bước này, sau khi được chọn lọc bởi local language model, top-k các candidate tiềm năng nhất tiếp tục được xếp hạng bởi global language model. Model được dùng làm global language model có thể nặng và có tốc độ phản hồi chậm nhưng cần có hiệu năng tốt nhất trong việc dự đoán next token, given the context. Sau đó, confidence score của mỗi candidate được tính bằng cách kết hợp local model, global model và các feature khác. Cuối cùng, 10 candidate có confidence score cao nhất được sử dụng làm kết quả gợi ý.


\subsubsection{Global language model}
\label{globallanguagemodel}
% Tại sao dùng global model
% Để thu được danh sách gợi ý phù hợp, mô hình được sử dụng để xếp hạng candidates cần có hiệu năng tốt nhất có thể. Tuy nhiên, this also comes at a price: mô hình có thể có kích thước nặng và tốc độ phản hồi chậm tính bằng giây, trong khi tốc độ gõ trung bình của lập trình viên là 1.47 giây/từ\cite{ase19}. Để khắc phục vấn đề này, chúng tôi triển khai mô hình như vậy làm global language model. Trong khi mỗi dự án đang được phát triển có một local language model tương ứng thì global language model được sử dụng chung cho tất cả dự án. Do đó, global model được huấn luyện trên một bộ dữ liệu lớn và có tính tổng quát hơn so với local model. Đồng thời, global model chỉ dự đoán một lượng giới hạn các candidates đã được chọn lọc bởi local model để giảm thời gian xử lý.

% Tại sao dùng GPT-2
% Cụ thể, chúng tôi sử dụng mô hình GPT-2\cite{gpt2} của OpenAI làm global language model. GPT-2 là một mô hình ngôn ngữ transformer-based đã được huấn luyện trên một bộ dữ liệu lớn gồm 40 GB dữ liệu văn bản của 8 triệu trang Web khác nhau. GPT-2 đạt điểm SOTA trên nhiều domain-specific language modeling tasks. GPT-2 cũng là core engine của công cụ Tabnine\cite{tabnine}.

% Dùng như thế nào
% GPT-2 vốn được phát triển để giải quyết các bài toán trong lĩnh vực xử lý ngôn ngữ tự nhiên. Mặc dù modeling code và model natural language might appear to be unrelated tasks, modeling code requires understanding natural language in some ways. Lí do là bởi mã nguồn cũng là dữ liệu dạng chuỗi (sequential data) và các từ khóa, định danh của nố thường sử dụng từ trong ngôn ngữ tự nhiên, hầu hết là Tiếng Anh. Thêm nữa, để huấn luyện lại từ đầu một mô hình GPT-2 mà đạt được hiệu năng cao cần rất nhiều thời gian và chi phí\cite{trainingcost}. Do đó, chúng tôi sử dụng mô hình pretrained có 345 triệu tham số được cung cấp bởi OpenAI. Chúng tôi tiến hành tinh chỉnh thêm trên bộ dữ liệu dạng mã nguồn bằng package gpt-2-simple[https://github.com/minimaxir/gpt-2-simple]. Mã nguồn của package đã được chỉnh sửa để mô hình có thể trả về likelihood mà một candidate là chuỗi theo sau một ngữ cảnh cho trước as the package only supports generating texts. GPU chúng tôi sử dụng cho quá trình huấn luyện và kiểm thử mô hình GPT-2 là Tesla P100.

\subsubsection{Preprocessing}
% Tiền xử lý dữ liệu
% Bộ dữ liệu mã nguồn được tiền xử lý trước khi được sử dụng để huấn luyện mô hình. Comments, annotations, blank lines and redundant indents are removed. Các literal kiểu String được làm rỗng vì chúng có thể chứa thông tin nhạy cảm. Đối với các biểu thức đối số phức tạp khó/không thể đoán như compound expressions và lambda expressions, các token đặc biệt <COMPOUND> và <LAMBDA> lần lượt tương ứng được chèn thêm phía trước. Nhờ vậy, ở pha dự đoán, mô hình dù có thể không đoán được cụ thể biểu thức vẫn có thể biết được kiểu biểu thức đối số.

% Khác với ngôn ngữ tự nhiên dạng văn bản (text), các khối khai báo phương thức trong mã nguồn có vai trò bình đẳng với nhau và không có quan hệ phụ thuộc trước sau/thuộc chứa. Do đó, mỗi khai báo phương thức (method declaration) trong mã nguồn nên được tách ra một văn bản (document?) riêng để tránh mô hình hiểu lầm rằng một phương thức được khai báo phía trước là precondition của phương thức được khai báo phía sau. Trong mỗi văn bản này, các thông tin về containing class (tên lớp, tên superclass, tên các superinterface), các khai báo trường (field declaration) và signature của các phương thức mà khối khai báo phương thức truy cập/gọi tới được thêm vào. Điều này giúp mô hình học được thông tin về kiểu dữ liệu của các trường, các phương thức, các tham số được sử dụng trong khối khai báo phương thức.
% Có cần thêm hình ví dụ?
% Ở pha dự đoán, ngữ cảnh của một Argument Recommendation Request cũng được xử lý tương tự, bao gồm khối khai báo phương thức (method declaration) trước vị trí truy vấn, thông tin về containing class và tất cả khai báo trường, method signatures của lớp đó.

\subsubsection{Selective Predicting}
% \label{selectivepredicting}
% Top-K candidates tiềm năng nhất được chọn lọc từ bước light ranking được gửi cho global model. The global model then re-evaluates their likelihood to be the next sequence following the coding context. To further decrease running time of \tool while maintaining good performance, only candidates of particular expression types, are re-evaluated. The chosen expression types should be the ones that the global model is the best at ranking. With regard to candidates of other expression types, their likelihood given the coding context are kept as they are in the light-ranking stage. Cụ thể, chúng tôi thử so sánh hiệu năng của hai mô hình nested-cached - our local model và GPT-2 - our global model trên mã nguồn của dự án Lucene[?]. Kết quả cho thấy GPT-2 performs tốt hơn ở cases mà expected argument expression types là Simple Name, Array Access, Type Literal, Object Creation, Array Creation, Lambda Expr, Method Reference. Trong khi đó, nested-cached performs tốt hơn đối với expected argument expression types còn lại. Do đó, the likelihood of a candidate $c$ given the coding context $P$ is re-evaluated as:
%
$$
\mathcal{P}(c,P)=
\begin{cases}
\mathcal{P}_{hr}(c,P) &\text{expr\_type(c)} \in \{ \} \\
\mathcal{P}_{lr}(c,P) &\text{Otherwise}
\end{cases}
$$
%
where $\mathcal{P}_{lr}(c,P)$ is evaluated by the light-weight LM and $\mathcal{P}_{hr}(c,P)$ is evaluated by the heavy-weight LM.

\subsubsection{Combining score}
Finally, given an AR request $r=\langle P, m\_call, pos \rangle$, the confidence score of a candidate $c$ is computed as:
$$
confidence\_score(c,r) = parasim(c,p) \times \mathcal{P}(c,P) \times p(dec(c,r)) \times p(use(c,r))
$$
where p(x) of a discrete random variable X is the probability that X equals to x.
Mười candidate có confidence score cao nhất được sử dụng làm kết quả gợi ý.

==> 5.empirical_method/5.2.procedure_bk.tex <==
\subsection{Evaluation Setup, Procedure, and Metrics}

Prior research~\cite{bigcode,curglm,ase19,PARC,nestedcache} has already investigated conducting code completion on benchmark datasets, especially on the task of argument recommendation~\cite{PARC}. To evaluate the performance of our proposed approach, we need to compare \tool against state-of-the-art methods. 

%

To the best of our knowledge, Asaduzzaman et al.~\cite{PARC} has proposed a technique, called PARC, which is currently the most effective technique for suggesting API method arguments. In fact, since PARC's implementation are not publicly accessible, we follow the their procedure to achieve benchmark dataset~\cite{PARC}, which is used to measure performance \tool against PARC.


%\textit{PARC defines a set of features to capture localness property of method parameters, which could be extracted from the code context prior to the suggesting position. Indeed, those features are all indexed into a large parameter usage database. For a new request of suggesting an argument, PARC searches similar usage from previous examples in the database and then lists the most likely argument candidates to developers.}

%
In addition, we employ nested cache model~\cite{nestedcache} to perform on AR task. This model is primarily built for code completion task, which learns from various code examples in order to predict next tokens from tokens come before it. To adapt nested cache model for predicting next argument, we need to combine multiple tokens to form a whole argument. Indeed, inpsired from previous work~\cite{bigcode}, while nested cache model making predictions, beam search algorithm is applied to find the \textit{k} highest probability sequences of tokens, which each of them corresponds to a complete argument.

%
We also compare our method with TabNine~\cite{tabnine}, a commercial code completion tool that has been widely used in the developer community. Since the core of TabNine is OpenAI's GPT-2 model~\cite{gpt2} which predicts next tokens based on the context, to measure performance of TabNine on AR task, we follow the same prediction procedure that applied for nested cache model.
%
\textit{[Which GPT-2 variant chose to reproduce the results]}. 
%Indeed, the following experiments will compare the performance of \tool and Tabnine on the same benchmark datasets of the argument recommendation task.



\begin{itemize}
    \item \textbf{Setup:}
    \begin{itemize}
        \item  Small: 10-fold for small
        \item Large: 400 projects for testing and the remaining for training
        \item  Static, dynamic, considering maintenance
    \item  Whole-Argument (WA)
    \end{itemize}
    \item \textbf{Procedure:} For each argument of every method call, split into 2 parts: context and target. (exactly match, standardize, e.g., this.p = p). 
    Given the project + context, predict rank accuracy
\end{itemize}
                    	
%
\textbf{Evaluation Setup:} We follow the same setting of splitting the dataset as in previous work of PARC~\cite{PARC} for the \textit{Small Corpus}. In particular, we divided all source files of \textit{Small Corpus} into 10 equal folds. To estimate performance of AR technique, we perform 10-fold cross-validation whereas each of the 10 folds is selected for testing and the remaining folds are used to train the AR model.

%
For the setting of \textit{Large Corpus}, we splitted 9,200 projects into 8,800 projects which are used as training data, while the remaining 400 projects are kept for testing purpose. Indeed, several projects in \textit{Large Corpus} cloned from Github are using old-version JAR libraries which no longer exist on public repositories. In consequence, AR techniques such as \tool, which explores all valid candidates by scanning information not only from program source code but also from external dependencies, cannot work as expected and might lead to missing target candidates in a huge number of cases. To avoid this problem, while choosing 400 projects for testing data, a prerequisite for those projects is all their dependencies are available, corresponding to the fact that the whole projects must be successfully compiled. 

%
\textbf{Testing Scenarios:}
To holistically measure the performance of AR approaches when they are incorporated into different coding scenarios, we adopt 3 test settings from existing work \cite{bigcode, nestedcache}, including \textit{Static}, \textit{Dynamic}, and \textit{Maintenance}. While the testing datasets are fixed through different settings, the training datasets differ as following:

\begin{itemize}
    \item \textit{Static tests:}. The model learns from a fixed training corpus and then perform predictions on the separate testing corpus for evaluating performance.
    \item \textit{Dynamic tests:} Instead of firmly restricting training corpus as in \textit{Static}, the model could iteratively update its parameters after each prediction on the source files of testing set. This setting comes from the idea that when developers need argument suggestions from AR tools, some source files are available at that time for dynamic adaptation. Note that, \tool contains 2 different models: \textit{Global Model} and \textit{Local Model}. Especially, while \textit{Local Model} could grow with information at test time, \textit{Global Model} is only trained on original training corpus and never adjusts its parameters after performing prediction.
    \item \textit{Software Maintenance tests:} The model, particularly \textit{Local Model} for \tool, could additionally learns from full test corpus except the file that is being tested. Although this setting requires the model to be retrained once per file in the test set, it can take full advantage of user source code at test time.
\end{itemize}
 
%
\subsection{Metrics} 
We report the performance of our approach on argument recommendation, which is the task of predicting a complete argument in a test corpus given the context of all the previous code tokens that extract from the beginning of containing method body to the recommending position. 

%
We adopted \textit{Precision}, \textit{Recall} and \textit{MRR} which are previously used in evaluating argument recommendation and code completion techniques~\cite{bigcode, nestedcache, PARC}.

\begin{equation}
Precision =\frac{relevant\; recommendations}{{supported\; recommendations}}
\end{equation}
\begin{equation}
Recall =\frac{relevant\; recommendations}{{ all\; recommendations}}
\end{equation}

In these two formulas above, \textit{all recommendations} denotes the total number of cases in test set. In fact, there are some of these cases that our approach cannot generate exact match candidates (e.g. compound expressions), so \textit{supported recommendations} is the number of cases that target arguments relating to expression types that \tool supports. Also, in prediction step, \textit{supported recommendations} shows number of cases that the target arguments are present in ordered lists of \textit{Top-k} suggestions generated by AR technique.

\begin{equation}
    MRR = \frac{1}{all\; recs} \sum_{i=1}^{all\; recs}{\frac{1}{rank_i}}
\end{equation}
\textit{[Rename all these terms (All recs) for shorter symbols?]}

%
In general, \textit{Precision} or \textit{Recall} represents whether the target arguments are presented in Top-k suggestion lists or not, which will be useful when developers need IDE to give most likely arguments instead of directly typing them. Meanwhile, \textit{Mean Reciprocal Rank (MRR)} focuses more on the rank of target argument in each suggestion list. For example, a MRR value of 0.5 shows that AR technique could suggest correct arguments at position 2 of ranked lists on average. In overall, the higher value of \textit{Precision} or \textit{Recall} or \textit{MRR} is, the better performance that AR techniques achieves.


==> 5.empirical_method/5.2.procedure_v1.tex <==
\subsection{Evaluation Setup, Procedure, and Metrics}

\textbf{Comparative  Study}.
To compare against the state-of-the-art approach in AR, PARC~\cite{PARC}, we applied the same setting and dataset. Specially, we randomly shuffled and divided the source files of each project in the \textit{small corpus} into 10 equal folds. We performed 10-fold cross-validation: each fold was chosen for testing, the remaining folds were used for training. For this setting, we also evaluated other baseline approaches: state-of-the-art $n$-gram LM with nested caching (SLP)~\cite{nestedcache} and representative deep neural network LM, GPT-2~\cite{gpt2}. GPT-2 is also the engine of TabNine which is one of the most popular AI-assisted completer~\cite{tabnine}.

%
However, SLP and GPT-2 are designed to predict next token for the given context. To adapt SLP and GPT-2 for AR task, we applied the same mechanism used in ~\cite{bigcode} to combine multiple predicted tokens to form a whole argument. Particularly, while predicting next tokens predictions, the beam search algorithm is applied to find the \textit{k} highest probability sequences of tokens, which each of them corresponds to a recommended argument.


We also evaluate \tool, SLP, and GPT-2 on the large corpus in three real-world AR scenarios~\cite{nestedcache}:
\begin{itemize}
    \item \textit{Static}. The model learns from a fixed training set and then perform recommending on the separate testing set for evaluating performance. In this scenario, we randomly used 400 projects for testing and the remaining for training.
%    
    \item \textit{Dynamic}. Instead of fixing the training set, the model could iteratively learn after each recommendation during testing. This setting comes from the idea that when developers need argument recommendations from tools, some source files are available at that time for dynamically learning. 
%
    \item \textit{Software Maintenance}. The approaches are tested on one file at a time in the test set. The approaches could learns from all the remaining files in test corpus. 
    % it can take full advantage of user source code at test time.
\end{itemize}

Since \textit{Software Maintenance} setting requires retraining once per file in the test set, this scenario has been shown that it is infeasible for DNN LMs~\cite{nestedcache} including GPT-2.
%
\tool contains 2 different models: \textit{Heavy-ranking stage} and \textit{light-ranking stage}. Especially, while \textit{light-ranking LM} could grow with information at test time, \textit{heavy-ranking Model} is only trained on original training corpus and never adjusts its parameters after performing prediction. \textbf{Something about privacy...}
%

\noindent \textbf{Intrinsic Analysis}.
%
We studied the impacts of the following components: valid candidate identification, candidate reduction, candidate ranking, and reducing size. We created different variants of \tool with different combinations and measured their performance.


\noindent \textbf{Sensitivity Analysis}. We studied the impacts of the following factors on the performance of \tool: training data size, context size, and origin of called methods. 
%

% \textbf{Evaluation Procedure.} From a source file of the test data, our evaluation tool traverses its code sequentially from the beginning. At a starting position \textit{pos} of an argument of a method call, we split the code sequence into 2 parts including a sequence of tokens start from containing method body to \textit{pos} (i.e., context) and the remaining tokens from \textit{pos} to the end position of this argument (i.e., actual argument). Based on the input context, AR tool computes \textit{top-k} most likely argument candidates. If the actual argument is among this k suggested candidates, we count this as a \textit{hit}. 

%
% 

%
\noindent \textbf{Metrics.} For comparison on the small corpus, we adopted the same metrics which are used in PARC~\cite{PARC}, \textit{Precision}, \textit{Recall}. Specially, $Precision(k) =\frac{R(k)}{S}$ and $Recall(k) =\frac{R(k)}{A}$, where $A$ is the total number of AR requests in test set, \textit{S} is the number of requests where the expression type of the expected argument is supported by \tool, and $R(k)$ is the number of requests where the recommended argument in top-k of the ranked list matches the expected one. Note that, for literals (e.g., string or number literals), \tool suggests the default values (e.g., "" or 0) and considers they matching the expected arguments since it might be impossible to suggest the actual values in these cases.
% \begin{itemize}
%     \item STRING\_LIT, CHAR\_LIT, NUM\_LIT -> normalize and do exact match
%     \item OBJECT\_CREATION, ARRAY\_CREATION, METHOD\_CALL -> match by \textit{startsWith}
%     \item CLASS\_EXPRESSION [.class] -> count as match if containing candidate = ".class" (not considering class name)
%     \item METHOD\_REFERENCE [.map(\textbf{Bicycle::new})] - 4 kinds of MethodRefs -> only match "::" %(https://docs.oracle.com/javase/tutorial/java/javaOO/methodreferences.html)
% \end{itemize}

For other experiments, we applied top-$k$ accuracy, and \textit{MRR} which are widely used in code completion~\cite{bigcode, nestedcache}. MRR is the average of reciprocal ranks for the test set:
$$
    MRR = \frac{1}{Q} \sum_{i=1}^{Q}{\frac{1}{rank_i}}
$$
%
% Also, in prediction step, \textit{supported recommendations} shows number of cases that the target arguments are present in ordered lists of \textit{Top-k} suggestions generated by AR technique.
%
% \textit{[Rename all these terms (All recs) for shorter symbols?]}
%
%
In general, top-$k$ accuracy represents whether the target arguments are presented in top-k ranked lists or not. 
Meanwhile, \textit{Mean Reciprocal Rank (MRR)} focuses more on the rank of target argument in each suggestion list. For example, a MRR value of 0.5 shows that AR technique could suggest correct arguments at position 2 of ranked lists on average.
% In overall, the higher value of \textit{Precision} or \textit{Recall} or \textit{MRR} is, the better performance that AR techniques achieves.


==> 6.empirical_result/tables/6.1.tab_comparison_argument_scope.tex <==
\begin{table}[]
\centering
\caption{Top-1 accuracy by argument scope on Large Corpus}
\label{tab:my-table}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{AutoAR} & \multicolumn{1}{c}{GPT-2} & \multicolumn{1}{c}{SLP} \\
 \midrule
Local argument & 89.81\% & 77.38\% & - \\
Others & 71.32\% & 37.16\% & - \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.1.tab_comparison_method_call.tex <==
\begin{table}[]
\centering
\caption{Top-1 accuracy by type of method call on Large Corpus}
\label{tab:my-table}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{AutoAR} & \multicolumn{1}{c}{GPT-2} & \multicolumn{1}{c}{SLP} \\
 \midrule
Intra method & - & - & - \\
Inter method & - & - & - \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.1.tab_comparison_small_topk.tex <==

\begin{table}[]
\small
\caption{Performance comparison in the \textit{general AR task} on the \textit{small corpus}}
\label{tab:small_corpus_top_k}
\centering
\begin{tabular}{@{}llccc@{}}
\toprule
Project & & \multicolumn{1}{c}{\tool} & \multicolumn{1}{c}{GPT-2} & \multicolumn{1}{c}{SLP} \\
\midrule
\multirow{5}{*}{Netbeans} & Top-1 & 65.15\% & 49.63\% & 34.91\% \\
 & Top-3 & 78.16\% & 56.98\% & 48.10\% \\
 & Top-5 & 81.10\% & 57.69\% & 55.02\% \\
 & Top-10 & 83.53\% & 57.87\% & 67.20\% \\\cmidrule(l){2-5}
 & \textit{MRR} & 0.72 & 0.53 & 0.44 \\
 \midrule
\multirow{5}{*}{Eclipse} & Top-1 & 64.19\% & 53.53\% & 28.52\% \\
 & Top-3 & 76.29\% & 61.18\% & 41.60\% \\
 & Top-5 & 79.23\% & 61.95\% & 49.46\% \\
 & Top-10 & 81.65\% & 62.10\% & 62.67\% \\\cmidrule(l){2-5}
 & \textit{MRR} & 0.70 & 0.57 & 0.38\\
 \bottomrule
\end{tabular}%
\end{table}


==> 6.empirical_result/tables/6.2.tab_intrinsic_global_model_eclipse.tex <==
\begin{table}[]
\centering
\caption{Intrinsic - Global Model (Eclipse)}
\label{tab:my-table}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{Top-1 (\%)} & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{Run. Time(s)} \\
 \midrule
GPT-2               & 64.19 & 0.70 & 0.402 \\
% nested cache & 69.35\% & 0.75 & 0.022 \\
RNN/LSTM                 & 25.60 & 0.44 & 0.182 \\
$n$-gram              & 36.30 & 0.47 & 0.146 \\
OFF    & 54.23 & 0.63 & 0.120 \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.2.tab_intrinsic_global_model_large_corpus.tex <==
\begin{table}[]
\centering
\caption{Intrinsic - Global Model (Large Corpus)}
\label{tab:my-table}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{Top-1 (\%)} & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{Run. Time(s)} \\
 \midrule
GPT-2               & 69.96 & 0.76 & 0.444 \\
% nested cache & 69.35\% & 0.75 & 0.022 \\
RNN/LSTM                 & - & - & - \\
$n$-gram              & 31.14 & 0.43 & 0.028 \\
OFF    & 69.35 & 0.75 & 0.022 \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.2.tab_intrinsic_global_model_netbeans.tex <==
\begin{table}[]
\centering
\caption{Intrinsic - Global Model (Netbeans)}
\label{tab:my-table}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{Top-1 (\%)} & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{Run. Time(s)} \\
 \midrule
GPT-2               & 70.71 & 0.76 & 0.732 \\
% nested cache & 69.35\% & 0.75 & 0.022 \\
RNN/LSTM              & 49.26 & 0.61 & 0.158 \\
$n$-gram              & 36.89 & 0.51 & 0.097 \\
OFF    & 65.37 & 0.72 & 0.085 \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.2.tab_intrinsic_local_model.tex <==
\begin{table}[]
\centering
\caption{Impact of Candidate Reduction on Performance}
\label{tab:intrinsic_cand_reduction}
\begin{tabular}{lccc}
\toprule
 & \multicolumn{1}{c}{Top-1} & \multicolumn{1}{c}{MRR} & \multicolumn{1}{c}{Run. Time(s)} \\
 \midrule
 
ON & 69.96\% & 0.76 & 0.444 \\
OFF & 61.98\% & 0.69 & 2.424 \\
\bottomrule
\end{tabular}%
\end{table}

==> 6.empirical_result/tables/6.3.tab_sensitivity_training_size.tex <==
\begin{table}[]
\centering
\caption{Sensitivity - Training data size (Small Corpus)}
\label{tab:my-table}
\begin{tabular}{lcc}
\toprule
 & Top-1 & MRR \\
 \midrule
1 fold & 63.78\% & 0.70 \\
3 folds & 65.97\% & 0.72 \\
5 folds & 66.86\% & 0.73 \\
7 folds & 67.45\% & 0.73 \\
9 folds & 67.67\% & 0.73 \\
\bottomrule
\end{tabular}
\end{table}
